Continuously monitored barrier options under Markov processes

In this paper we present an algorithm for pricing barrier options in one-dimensional Markov models. The approach rests on the construction of an approximating continuous-time Markov chain that closely follows the dynamics of the given Markov model. We illustrate the method by implementing it for a range of models, including a local Levy process and a local volatility jump-diffusion. We also provide a convergence proof and error estimates for this algorithm.

==> StateSpace.tex <==
%We are going to present some numerical results to demonstrate the accuracy
%of our method. First of all, we need to define an algorithm to generate a
%non-uniform grid. 
%which was
%used in Section~\ref{sec:numerical}
%to approximate the Markov process 
%$S$.
%A widely used method for generating a non-uniform state-space consists of 
%applying a coordinate transformation to a uniform state-space, which is what we will
%do.
The algorithm for constructing a non-uniform grid 
$\{x_1,\ldots,x_N\}$
with 
$N\in2\NN$
points
for the triplet
$a<s<b$
with density parameters
$g_1$
and
$g_2$
is given by the following procedure.
\begin{enumerate}
\item Compute $c_1 = \mathrm{arcsinh}\left(\frac{a-s}{g_1} \right)$, 
           $c_2 = \mathrm{arcsinh}\left(\frac{b-s}{g_2} \right)$.  
	  % $N_a = \lceil N/2\rceil$ and $N_b = N-(N_a+1)$.
%\item Generate a uniform grid $y\in[0,1]$ with $N_l$ number of points.
\item Define the lower part of the grid by the formula
      $x_k := s + g_1 \mathrm{sinh}(c_1(1-(k-1)/(N/2-1)))$
      for 
      $k\in\{1,\ldots,N/2\}$.
      Note that $x_1=a, x_{N/2}=s$.
%\item Generate a uniform grid $y\in[0,1]$ with $N_u$ number of points.
\item Define the upper part of the grid using the formula
      $x_{k+N/2} := s + g_2 \mathrm{sinh}(c_2 2k/N)$
      for 
      $k\in\{1,\ldots,N/2\}$.
      Note that 
      $ x_{N}=u$.
%\item Define the non-uniform lattice by concatenating 
%      the lower and upper parts given in (3)~and~(4). 
\end{enumerate}

The 
non-uniform state-space 
$\GG\subset\E$
for the Markov chain
$X$, 
used for the pricing of a double-barrier option 
with barrier levels
$l<u$,
can now be constructed in the following way.
Pick
$N\in3\NN$,
choose the smallest  
$x_1$
and largest 
$x_N$
values of the grid
$\GG$
and apply the procedure above three times to the triplets
$x_1<l<(s-l)/2$,
$(s-l)/2<s<(u-s)/2$
and
$(u-s)/2<u<x_N$,
each time with 
$N/3$
points and some density parameters. 
The state-space 
$\GG$
is obtained by concatenating the three grids
(see also the Matlab function that generates this
grid in~\cite{MG_Code}).







==> barrier_time3.tex <==
In practical applications model parameters such as the 
short rate or the volatility function are often taken to be 
time-dependent. In this section we will briefly show how the 
results of the earlier section can be adapted to this 
time-dependent setting. 

We now start from a time-inhomogeneous Markov process 
$S = \{S_t\}_{t\in[0,T]}$, 
modelling the evolution 
the risky asset price under consideration until some maturity $T>0$. 
Then the time-space process 
$\{(t,S_t)\}_{t\in[0,T]}$ 
forms a two-dimensional homogeneous Markov process, and the approach
developed in
Section~\ref{sec:barrier_MP} can 
be easily adapted to this case, which we now outline.
To highlight the role of time as a factor we denote by 
$D=\{D_t\}_{t\geq0}$ 
and
$Y=\{Y_t\}_{t\geq0}$ 
where
\begin{eqnarray}
\label{eq:DefY_D}
D_t:=(D_0 + t)\wedge T\qquad\text{and}\qquad
Y_t := S_{D_t}\quad\forall t\geq0.
\end{eqnarray}
Then, for any $s,t>0$  and
bounded Borel function $f:[0,T]\times \E\to\RR$ 
it holds that
\begin{equation*}
\EE[f(D_t,Y_t)|\mathcal F_s] = (Q_tf)(D_s, Y_s),
\end{equation*}
where
\begin{eqnarray*}
(Q_t f)(s,x) &=& \EE_{s,x}[f(D_t, Y_t)] := \EE[f(D_t,Y_t)|D_0=s,Y_0=x]\\
&=& \EE[f(s+t,S_{(s+t)\wedge T})|S_s=x].
\end{eqnarray*}
Thus the family $(Q_t)_{t\ge 0}$ forms a (two-dimensional) semigroup.
We will restrict ourselves to the case when 
$(D,Y)$ 
is a Feller 
process with state-space $\E':=[0,T]\times \E$, in the sense of 
Assumption~\ref{def:Feller} with $\E$ replaced by $\E'$. 
Associated to the semigroup $(Q_t)_{t\geq0}$ is the infinitesimal generator
${\mc L}'$ defined by
\begin{equation*}
\lim_{t\downarrow 0} t^{-1} [Q_tf(s,x) - f(s,x)] = {\mc L}'f(s,x),
\end{equation*}
for all $f$ in the set ${\mc D}'$, the domain of $\mc L'$, 
for which this limit exists. The process stopped upon entering a 
closed set $A$ remains a Markov process, and 
its corresponding generator 
can be obtained as in Section \ref{sec:barrier_MP}.
Denote by $\mathcal L_t$ the generator restricted to functions 
$g:\E\to\mathbb R$ of space only, that is,
$(\mathcal L_tg)(x) := (\mathcal L'g)(t,x)$.

We next give two examples of models in which
time-dependence plays a natural role --- we will present a numerical 
illustration of these models in Section \ref{sec:numericalEx}.

\begin{Ex}\label{ex:dupire}
\rm
Given a surface of arbitrage-free call option prices generated by 
some diffusion model, there exists a one-dimensional diffusion 
with time-dependent volatility function
$\Sigma(t,x)$ 
that reproduces those 
option prices. 
The volatility function 
$\Sigma(t,x)$ 
is explicitly given in terms of the call option prices 
by Dupire's formula. 
In such a local volatility model the stock price 
$S=\{S_t\}_{t\in[0,T]}$ evolves according
to the SDE
\begin{equation}\label{eq:locvol}
\td S_t = \gamma(t,S_t)\td t + \Sigma(t,S_t)\td W_t,
\end{equation}
where $\gamma(t,x) = (r(t)-d(t))x$ with 
$r(t)$ and $d(t)$ continuous functions representing 
the interest and dividend rate, and $\Sigma(t,x)$ is a 
volatility function chosen sufficiently regular that 
$\{(D_t,Y_t)\}_{t\geq0}$ is a Feller process and the 
discounted stock price 
$\{\te{-\int_0^t[r(s)-d(s)]\td s}S_t\}_{t\in[0,T]}$ is a martingale.  
The corresponding infinitesimal generator   
then acts on functions $f\in C^{2}_c(\mathbb E)$ as
\begin{equation*}%\label{eq:gen.localvol}
({\mc L}_tf)(x) =  
\gamma(t,x)\nabla f(x) + \mbox{$\frac{1}{2}$}
\Sigma^2(t,x)\Delta f(x),
\end{equation*}
 where
$\nabla f, \Delta f$ denote 
the first and second derivatives with respect to $x$.
%$\sigma(t,x)$ is strictly positive for $t,x>0$, and continuous as
%function of $(t,x)$.
\end{Ex}

\begin{Ex}\label{eq:additive}
\rm
In an exponential additive model the log-price is a spatially
homogeneous Markov process, and $S=\{S_t\}_{t\in[0,T]}$ is given by
\begin{equation}\label{eq:expadd}
S_t = \te{\int_0^t[r(s) - d(s)]\td s}\ S_0\frac{\te{X_t}}{\EE_0[\te{X_t}]},
\end{equation}
where $X$ is an {additive} process, a process with 
independent increments and cadlag paths. If $\EE[\te{X_t}]<\infty$ 
for all $t\in[0,T]$, the discounted process 
$\{\te{-\int_0^t[r(s)-d(s)]\td s}S_t\}_{t\in[0,T]}$ is a martingale, by construction.

To be specific, let $X$ be an additive process $X=\{X_t\}_{t\in[0,T]}$ 
with drift and volatility functions $\beta(t)$ and $\sigma(t)$, and 
a system of 
L\'{e}vy measures 
$\nu(t,\td y)$, given by
\begin{equation}\label{eq:addreg}
X_t = \int_0^t\beta(s)\td s + \int_0^t\sigma(s)\td W_s +
Z_t.
\end{equation}
Here the process
$Z=\{Z_t\}_{t\in[0,T]}$ 
is a jump-process with compensator 
$\nu(t,\td y)\td t=g(t,y)\td y\td t$ satisfying 
the integrability condition 
\begin{equation}\label{eq:intadd}
\int_{\mathbb R\backslash\{0\}}(1\wedge y^2) \sup \{g(s,y):s\in[0,T]\}\>\td y<\infty, \end{equation} 
with 
%$\beta$, $\sigma: [0,T]\to\RR$ and 
$g(\cdot,y):[0,T]\to\RR_+$, $y\in\mathbb R\backslash\{0\}$, 
a family of continuous functions. 
Models from this class (with $\sigma\equiv0$ and a particular form of 
$g(t,y)$) have been proposed for stock price modelling by Carr et al. 
\cite{CarrMadanGemanYor_selfdec} --- see also 
Section \ref{subsub:Sato}. 
%
%\begin{comment}
%For any $t\in[0,T]$, the distribution of $X_t$ is infinitely divisible, %with
%characteristic function $\Phi_t(z)=\exp(\ovl\Psi_t(z))$  given in terms% %
%of the characteristics by
%$\ovl\Psi_t(z)=\int_0^t\Psi_s(z)\td z$ where
%$$
%\Psi_s(z) = \mathtt i \beta(s) z - \frac{\sigma^2(s)}{2} z^2 +
%\int_{\mathbb R}[\te{\mathtt i z y} - 1 - \mathtt i
%zy1_{\{|y|<1\}}]g(s,y)\td y.
%$$
%\end{comment}
Then the time-space process $\{(D_t,Y_t)\}_{t\geq0}$ is a Feller process, 
with an infinitesimal generator acting on $f\in C^{2}_c(\mathbb E)$ 
as\footnote{A proof of these facts is given in Appendix~\ref{sec:proofs}.}
\begin{eqnarray}\label{eq:gen.add}
(\mc L_tf)(x) &=& (\mc L^cf)(t,x) + \int_{\RR} 
\le[f(x\te{y}) - f(x) 
- \nabla f(x)x(\te{y}-1)\I_{\{|y|<1\}}\ri]g(t,y)\td y,\\ 
(\mathcal L^c f)(t,x) 
&:=& \WT\beta(t)x\nabla f(x) + \frac{\sigma^2(t)}{2}x^2 \Delta f(x),\nonumber
%\label{eq:cont.gen.add}
\end{eqnarray}
%is the generator 
%of a geometric Brownian motion with infinitesimal drift $\WT\beta(t)$ 
%and volatility $\sigma(t)$. 
where $$\WT\beta(t) = 
r(t)-d(t)  - 
\int_{\mathbb R}(\te{y} - 1)\I_{\{|y|>1\}}g(t,y)\td y.$$
\end{Ex}

\subsection{Time-inhomogeneous chains}
To approximate
the barrier option prices driven by a given 
time-inhomogeneous Markov process we again start 
by constructing an appropriate Markov chain. 
%
%
% The idea is to approximate the time-dependent model of 
% interest by taking the parameters to be piecewise constant in time,
% and apply inductively Theorem~\ref{thm:Main}: the barrier option 
% value is then obtained by matrix multiplication.
%
We build an approximating
time-inhomogeneous chain with a generator that is 
piecewise constant in time. Given a partition 
$\mathbb T = \{T_i\}_{i=0}^n$ with
$T_0=0<T_1<\ldots<T_n=T$ of $[0,T]$, we assume that the chain $X$ 
on the state-space $\mathbb G$ evolves according to the 
generator $\Lambda^{(i)}$ during the time-interval $[T_{i-1}, T_{i})$
where the matrices $\Lambda^{(i)}$ are chosen so as to approximate 
well the 
infinitesimal generators $\mathcal L_{T_i}$.
Thus $X$ has a time-dependent generator given by
\begin{equation}\label{eq:GeneratorTimeDep}
\L_t:=\sum_{i=1}^{n}\L^{(i)} \I_{[T_{i-1},T_i)}(t),\qquad t\geq0.
\end{equation}
%with $T_{n+1}=\infty$. 
%
% We build an approximating
% time-inhomogeneous chain with a generator that is a 
% piecewise constant in time. Given a partition 
% $\mathbb T = \{T_i\}_{i=0}^n$ with
% $T_0=0<T_1<\ldots<T_n=T$ of $[0,T]$, we assume that the chain $X$ 
% on the state-space $\mathbb G$ evolves according to the 
% generator $\Lambda^{(i)}$ during the time-interval $[T_i, T_{i+1})$
% where the matrices $\Lambda^{(i)}$ are chosen so as to approximate 
% well the 
% infinitesimal generators $\mathcal L_{T_i}$.
% Thus $X$ has a time-dependent generator given by
% $$
% \L_t:=\sum_{i=1}^{n+1}\L^{(i)} \I_{[T_{i-1},T_i)}(t),\qquad t\geq0,
% $$
% with $T_{n+1}=\infty$. 
Also we take the short rate 
$r^{(n)}$
to be piecewise constant
\begin{equation}\label{rd}
r^{(n)}(t) = \sum_{i=1}^{n}r_i\,\I_{[T_{i-1},T_i)}(t),\qquad 
%d^{(n)}(t) = \sum_{i=1}^{n+1}d_i\,\I_{[T_{i-1},T_i)}(t),
\text{for}\>\>
t\geq0\>\>
\text{and}\>\>
r_i\geq0,\> i=1,\ldots,n.
\end{equation}
As a straightforward consequence of Theorem~\ref{thm:Main}
we have the following result for the first-passage probabilities
of the chain $X$.

\begin{Cor}
\label{cor:TimeDep}
For $r^{(n)}$ given as above and any functions 
$\phi:\WH{\mathbb G}\to\mathbb R$ and 
$\psi:\mathbb G\to\mathbb R$ 
with $\psi(x)=0$ for $x\in\WH\E$,
the following equalities hold
\begin{eqnarray}
\EE_x\left[\phi(X_T)\I_{\{\tau>T\}}\right]
& = & \left(\exp\left(\Delta T_1\WH\L^{(1)}\right)
\cdots
\exp\left(\Delta T_n\WH\L^{(n)}\right)\phi\right)(x),
\quad x\in\WH{\mathbb G},
\label{eq:BarrierTimeDep}\\
\qquad\EE_x\left[\te{-\int_0^\tau r^{(n)}(t)\td t}\psi(X_\t)\I_{\{\tau\leq T\}}\right]
& = & \left(\exp\left(\Delta T_1\WT\L^{(1)}_{r_1}\right)
\cdots
\exp\left(\Delta T_n\WT\L^{(n)}_{r_n}\right)\psi\right)(x),
\quad x\in\mathbb G,
\label{eq:BarrierTimeDep2}
\end{eqnarray}
where $\Delta T_i:=T_i-T_{i-1}$,
and $\WH\L^{(i)}$ and $\WT\L^{(i)}_{r_i}$ are defined 
as in~\eqref{eq:Def_tA} and \eqref{eq:Def_tilA}.
\end{Cor}


% We also take the short and dividend rates $r$ and $d$ to be piecewise constant,
% \begin{equation}\label{rd}
% r(t) = \sum_{i=1}^{n+1}r_i\,\I_{[T_{i-1},T_i)}(t),\qquad d(t) = \sum_{i=1}^{n+1}d_i\,\I_{[T_{i-1},T_i)}(t),
% \qquad t\geq0.
% \end{equation}
% As a straightforward consequence of Theorem~\ref{thm:Main}
% we have the following result for prices of barrier options driven by $X$:
% 
% \begin{Cor}
% \label{cor:TimeDep}
% For $r$ given as above and any functions 
% $\phi:\WH{\mathbb G}\to\mathbb R$ and 
% $\psi:\mathbb G\to\mathbb R$ 
% with $\psi(x)=0$ for $x\in\WH\E$,
% the following equalities hold
% \begin{eqnarray}
% \EE_x\left[\te{-\int_0^T r(t)\td t}\phi(X_T)\I_{\{\tau>T\}}\right]
% & = & \left(\exp\left(\Delta T_1\WH\L^{(1)}_{r_1}\right)
% \cdots
% \exp\left(\Delta T_n\WH\L^{(n)}_{r_n}\right)\phi\right)(x),
% \quad x\in\WH{\mathbb G},
% \label{eq:BarrierTimeDep}\\
% \EE_x\left[\te{-\int_0^\tau r(t)\td t}\psi(X_\t)\I_{\{\tau\leq T\}}\right]
% & = & \left(\exp\left(\Delta T_1\WT\L^{(1)}_{r_1}\right)
% \cdots
% \exp\left(\Delta T_n\WT\L^{(n)}_{r_n}\right)\psi\right)(x),
% \quad x\in\mathbb G,
% \label{eq:BarrierTimeDep2}
% \end{eqnarray}
% where $\Delta T_i:=T_i-T_{i-1}$
% and $\WH\L^{(i)}_{r_i}$ and $\WT\L^{(i)}_{r_i}$ are defined 
% as in~\eqref{eq:Def_tA} and \eqref{eq:Def_tilA}.
% \end{Cor}
% 

%Note that expression~\eqref{eq:BarrierTimeDep}
%directly translates into an algorithm for the pricing
%of barrier options in models with time dependent coefficients.
%The number
%$n$
%in Corollary~\ref{cor:TimeDep}
%is in practice not very large
%(say around 10)
%because the parameters of the model are taken to be constant
%between market defined maturities
%for which the prices of
%liquid options
%can be observed.
%The pricing algorithm in the time dependent case is
%linear in the number of time intervals
%$n$
%and
%$n$
%additional matrix-matrix multiplications make only marginal difference
%compared to the time independent case.
%
%Note that Eq.~\eqref{eq:BarrierTimeDep}
%encompasses an approximation European option price in the model $X$
%with time dependent coefficients by taking $\WH{\G}=\G$, which leads to
%$$
%\EE_x\left[\te{-\int_0^T r(t)\td t}\phi(X_T)\right]  =  
%\left(\exp\left(\Delta T_1\L_{r_1}^{(1)}\right)
%\cdots \exp\left(\Delta T_n\L_{r_n}^{(n)}\right)\phi\right)(x).
%$$








